Normal basises and symbolical dynamics

The thesis is devoted to relations between algebra and symbolic dynamics. Various generalisations of sturmian sequences are discoursed. Let $W$ be an infinite word over a finite alphabet $A$. The combinatorial criteria of existence of interval exchange transformations that generate the word $W$ is obtained in full generality -- no IDOC condition assumed, case of orientation non-preserving also considered.

==> bib_old.tex <==
\begin{thebibliography}{MH1}

\bibitem{NA} С.И. Адян. Проблема Бернсайда и тождества в группах // М., Наука,
1975.

\bibitem{B1} А.Я.Белов, Классификация слабо нетеровых мономиальных
алгеб // Фунд. и прикл. мат. -- 1995.--1.,б4, --С. 1085-1089.

\bibitem{BBL} А.Я.Белов, В.В.Борисенко, В.Н.Латышев, Мономиальные
алгебры // Итоги науки и техники.Совр. Мат. Прил. Тем. Обзоры т.
26 (алг. 4), М. 2002. 35-214.

\bibitem{BK} А.Белов, Г.Кондаков, Обратные задачи символической
динамики // Фундаментальная и прикладная математика, Т1, №1, 1995


\bibitem{Kol} А.Т. Колотов, Апериодические последовательности и функции роста в
алгебрах // Алгебра и логика, 20 (1981), 138-154, 250.

\bibitem{Kol} А.Т. Колотов, Алгебры и группы с периодической
функцией роста // Алгебра и логика, 19 (1980), 659-668, 745.


\bibitem{LSh} Р.Линдон ,П.Шупп, Комбинаторная теория групп // М.,
Мир, 1980.

\bibitem{Sin} Я.Г. Синай, Введение в эргодическую теорию // М.: ФАЗИС, 1996. 144 с.   

\bibitem{Uf} Уфнаровский В.А. Комбинат. и асимпт. методы в алгебре. // Итоги
науки и тех. Серю Совр. Пробл. Мат. Фунд. направл. М. ВИНИТИ.
1990- 57, стр 5-177. (РЖМат, 1990).

\bibitem{Ab} A.Aberkane, Words whose complexity satisfies $\lim p(n)/n
= 1$ // Theor. Comp. Sci., 307, (2003), 31-46.

\bibitem{AR} P. Arnoux and G. Rauzy [1991],
Representation geometrique des suites the complexite $2n + 1$ //
Bull. Soc. Math. France 119, 199-215.

\bibitem{BG} A.Belov, Т. Gateva-Ivanova, Radicals of monomial
algebras // Proceedings of Taiwan-Moscow Algebra Workshop, -- C.
159-169.

\bibitem{Belov} A. Belov.
Some estimations for nilpotence of nil-algebras over a field of an
arbitrary characteristic and height theorem // {\it Communications
in algebra}, 20 (10):2919-2922, 1992.

\bibitem{Be} G.M. Bergman, A note on growth functions of
algebras and semigroups // Research Note, University of
California, Berkeley, 1978.


\bibitem{BS} J. Berstel, P. S\'{e}\'{e}bold, Sturmian words, in: M. Lothaire (Ed.) // Algebraic Combinatorics on Words,
Encyclopedia of Mathematics and Its Applications, Vol. 90,
Cambridge University Press, Cambridge, 2002 (Chap. 2).

\bibitem{B} J.Berstel, Resent results on Sturmian words //
Developments in language theory II, 13-24, World Scientific, 1996.

\bibitem{DP} X. Droubay, G. Pirillo, Palindromes and sturmian
word// Theroret. Comput. Sci., 223:73-85, 1999.

\bibitem{DJP} X.Droubay, J.Justin, G.Pirillo, Episturmian words
and some construction of de Luca and Rauzy // Theoret. Comp.
Sci.,2000, to appear.


\bibitem{F}H. Furstenberg. Poincar\'e reccurence and number
theory // Bull. Amer. Math. Soc., 5:211-234, 1981.


\bibitem{GR} R. L. Graham, Covering the Positive Integers by disjoints sets of the form $\{[n\alpha + \beta]: n=1, 2,
\ldots\}$ // J. Combin. Theory Ser A15 (1973) 354-358.

\bibitem{H} P. Hubert, Well balanced sequences // Theoret. Comput. Sci. 242 (2000) 91–108.


\bibitem{KL}Krause, G.; Lenagan, T.H.: Growth of algebra and
Gelfand-Kirillov dimension // Research Notes in Math., Pitman,
London, 1985.

\bibitem{AdL} A. de Luca, Sturmian words: structure,
combinatorics and their arithmetics // Theoret. Comp. Sci., 183,
(1997), 45-82.

\bibitem{DV1} A. de~Luca and S. Varricchio.
Combinatorial properties of uniformly recurrent words and an
application to semigroups. // {\it Inter. J. Algebra Comput.},
1(2):227--246, 1991.MR 92h:20084.


\bibitem{L1} M. Lothaire, Combinatorics on Words // Encyclopedia of
Mathematics and its Applications, Addison-Wesley, Reading, MA,
1983, Vol. 17.

\bibitem{L2} M. Lothaire, in: J. Berstel, P. S\'e\'ebold (Eds.) // Algebraic Combinatoric on Words, Ch. 2: Sturmian
Words, Cambridge Univ. Press, to appear.


\bibitem{MorseHedlund} M. Morse and G. A. Hedlund [1940], Symbolic dynamics II.
Sturmian trajectories, // Amer. J. Math. 62, 1-42.


\bibitem{Ra} G. Rauzy,
Mots infnis en arithmetique, in: Automata on Infnite Words //
Ecole de Printemps d'Informatique Thfeorique, Le Mont Dore, May
1984, ed. M. Nivat and D. Perrin, Lecture Notes in Computer
Science, vol. 192, Springer-Verlag, Berlin etc., pp. 165-171, 1985

\bibitem{Ra2} G. Rauzy, Suites \'a termes dans un alphabet fini //
In {\it S\'emin. Th\'eorie des Nombres,} p. 25-01-25-16,
1982-1983, Expos\'e No 25.

\bibitem{RS} G. Rozenberg and A. Salomaa //
The Mathematical Theory of L Systems, Academic Press, New York
etc., 1980

\bibitem{R} G.Rote, Sequences with subword complexity $2n$ // J. Number Theory 46 (1994) 196–213.

\bibitem{Sal81}
Arto Salomaa.{\it Jewels of Formal Language Theory} // Computer
Science Press, 1981.

\bibitem{T1}R.Tijdeman, Decomposition of the integers as a
direct sum of two subsets // in: Number Theory, ed. by S. David, Number Theory Seminar Paris 1992-93, Cambridge University Press, (1995), 261-276

\bibitem{T2}R.Tijdeman, Fraenkel's conjecture for six
sequences // Discrete Mathematics, Volume 222,  Issue 1-3, 223 - 234, 2000
 
\bibitem{V} L. Vuillon, Balanced words // Bull. Belg. Math. Soc. Simon Stevin 10 (2003), no. 5, 787-805

\bibitem{V2} L.Vuillon, A characterization of Sturmian word by
return words // European Journal of Combinatorics (2001) 22, 263-275.


\bibitem{W} H.Weyl, \"{U}ber der gleichverteilung von zahlen mod
1, // Math. Ann., v. 77, 313-352, 1916.


\end{thebibliography}


==> chapter3_dop.tex <==
\subsection{Случай одной двойной развилки.}

Покажем теперь, как этот подход работает в случае минимального
роста.


Поскольку $2$-слов ровно на одно больше, чем $1$-слов, то это
значит, что при отображении $T^{-1}$ количество интервалов
разбиения увеличилось ровно на $1$. Это означает, что $I^1$
отличается от $I^0$ всего  одной точкой,которая делит
характеристическое множество, соответствующее правому специальному
$1$-слову,на два интервала.


Однако вспомним, что вариант $a)$ (см. Рис.) в случае одной развилки
соответствуют нерекуррентному слову, а потому невозможны. В  случае
нескольких развилок эти варианты учитывать нужно.


В общем случае, так как ($k+1$)-cлов на $1$ больше, чем $k$-слов,
то $I^{k}$ добавляет к $I^{0}\cup I^1\cup \ldots \cup I^{(k-1)}$
одну новую точку, которая делит правое специальное $k$-слово на
два интервала, соответствующие двум его продолжениям.

\subsection{Случай двух и более двойных развилок.}

Аналогично случаю с одной развилкой, так как $2$-слов ровно на $k$
больше, чем $1$-слов, то это значит, что при отображении $T^{-1}$
количество интервалов разбиения увеличилось ровно на $k$. Это
означает, что $I^1$ отличается от $I^0$ ровно $k$ точками,которые
делят характеристическое множество, соответствующее правому
специальному $1$-слову,на $k+1$ интервал.


В общем случае, так как ($k+1$)-cлов на 1 больше, чем $k$-слов, то
$I^{k}$ добавляет к $I^{(0)}\cup I^1\cup \ldots \cup I^{(k-1)}$ одну
новую точку, которая делит правое специальное $k$-слово на два
интервала, соответствующие двум его продолжениям.


==> intro_old.tex <==
\section{Введение.}
\subsection{Актуальность темы}
Комбинаторика слов находится на стыке алгебры и теории динамических
систем.


Комбинаторика слов широко используется  в задачах комбинаторной
теории групп (\cite{LSh},\cite{NA}), в теории алгебр Ли, вопросах
бернсайдовского типа (Ширшов) и задачах, связанных с мономиальными
алгебрами.

Комбинаторная техника, относящаяся к теории групп, развивалась в
работах М.~Дэна, Е.~И.~ Голода и И.~Р.~ Шафаревича, П.~С.~
Новикова, С.~И.~ Адяна, И.Рипса, А.~Ю.~Ольшанского.

В теории алгебр Ли описание базиса дается в терминах так
называемых ``правильных слов'' (базис Холла-Ширшова).

С помощью комбинаторики слов А.И. Ширшов доказал теорему о свободе
подалгебры свободной алгебры Ли. Для супералгебр это обобщил А.А.
Михалев. Он показал алгоритмическую разрешимость проблемы
равенства для алгебр ли с одним определяющим соотношением.

Комбинаторика слов активно используется в проблемах
бернсайдовского типа, в теории $PI$-алгебр, достаточно упомянуть
теорему Ширшова о высоте.


Также техника комбинаторика слов работает в теории полугрупп.
Здесь можно упомянуть работы М.~В.~ Сапира, О.~Г.~ Харлампович.

Понятие {\it роста} в алгебре является важным комбинаторным
инвариантом, ему посвящена монография \cite{BBL}, \cite{KL}.
Обобщение понятия роста на бесконечномерный случай является понятие
{\it ряда коразмерностей}, введенное А.Регевым. Первоначальное
доказательство А.Регева об экспоненциальной оценке ряда
коразмерности относительно свободных алгебр было улучшено В.~Н.~
Латышевым с помощью числа полилинейных $n$-разбиваемых слов на
основе теоремы Дилуорса.

Ряды коразмерности исследовались также в работах В.Н. Латышева,
С.П. Мищенко, М.В. Зайцева, A.Giambruno.


Вопросы, связанные с мономиальными алгебрами, приводят  изучению
бесконечных (в одну или обе стороны) слов или {\it сверхслов}.
Фундаментальным понятием в теории сверхслов является понятие {\it
равномерно-реккурентного} слова, введенное Фюрстенбергом \cite{F}.
Слово $W$ называется {\it равномерно-реккурентным}, если для
каждого подслова $v\subset W$ существует натуральное $N(v)$,
такое, что для любого подслова $u\subset W$  длины не менее, чем
$N(v)$, $v$ является подсловом $u$.

Имеет место следующая \par {\bf Теорема}. Пусть $W$ -- бесконечное
сверхслово. Тогда существует такое равномерно-реккурентное слово
$\hat{W}$, все подслова которого являются подсловами $W$.

Эта теорема исключительно важна в комбинаторике слов, поскольку
очень часто позволяет свести изучение произвольных слов к изучению
равномерно-рекуррентных слов.

В терминах равномерно-рекуррентных слов строится теория радикалов
мономиальных алгебр. Мономиальная алгебра называется {\it
мономиально почти простой}, если фактор по идеалу, порожденному по
любому моному, нильпотентен.

Множество ненулевых слов в почти простой мономиальной алгебре есть
множество всех подслов некоторого равномероно-рекуррентного слова.

Пересечение же идеалов с почти простым фактором совпадает с
нильрадикалом мономиальной алгебры, а также ее радикалом
Джекобсона (см. \cite{BG}).


В терминах равномерно-рекуррентных слов также получается описание
слабо нетеровых мономиальных алгебр. Каждое ненулевое слово слабо
нетеровой мономиальной алгебры есть подслово из набора
(сверх)слов, удовлетворяющего следующему условию: каждое слово из
этого набора либо конечное, либо является бесконечным
(односторонними или двухсторонними) словом, которое при
выбрасывании некоторого конечного куска распадается на
равномерно-рекуррентные части.

Существует разные подходы к изучению сверхслов:

\begin{enumerate}
\item Непосредственно комбинаторные свойства слов

\item Графы подслов, или {\it графы Рози}

\item Топологическая динамика
\end{enumerate}

%Библиография по общей теории слов.
Классическими работами по теории комбинаторики слов являются
монографии \cite{L1,L2}, \cite{RS}.

%Графы Рози.
Другим инструментом изучения сверхслов является понятие графов
подслов или {\it графов Рози}. Если $W$ -- бесконечное сверхслово
над алфавитом $A$, то {\it $k$-графом Рози} называется граф,
вершины которого соответствуют различным подсловам $W$ длины $k$.
Из вершины $w_1$ в вершину $w_2$ ведет стрелка, если максимальный
суффикс $w_1$ совпадает с максимальным префиксом $w_2$, то есть
$w_1=a_1u$, $w_2=ua_2$, где $a_1,a_2 \in A$.

Общий подход, связанный с описанием слов с помощью динамических
систем, следующий.  Пусть $W=\{w_n\}$ -- бесконечное слово. $\tau
(\{w_n\})=\{w_{n+1}\}$ -- оператор сдвига. Рассмотрим замыкание
траектории слова относительно метрики Хэмминга $X \in A^*$. Прямые
задачи символической динамики связаны с получением информации о
динамической системе $(X,\tau)$ по информации о слове $W$.

Известно, что если слово $W$ {\it равномерно-рекуррентно}, то
полученная динамическая система минимальна, то есть не содержит
нетривиальных замкнутых инвариантных траекторий.

Также стоит отметить работу  \cite{BK}, изучающую слова,
получаемые из взятия дробных частей многочленов со старшим
иррациональным коэффициентом в целых точках.

Обратно, пусть имеется дискретная топологическая динамическая
система, то есть задано компактное топологическое пространство
$M$, гомеоморфизм $f:M\to M$ и несколько открытых подмножеств
$U_1,U_2,\ldots U_{n-1}$. Положим также $U_n=M \setminus U_1\cap
U_2\cap \ldots \cap U_{n-1}$. Рассмотрим начальную точку $x \in M$
и последовательность итераций $f^{-1}(x),x,f(x),\ldots$. По этой
последовательности можно построить слово $W=\{w_n\}$ над алфавитом
$A=\{a_1,a_2,\ldots a_n\}$ следующим образом: $w_i=a_k$, если $f^i
\in U_k$. По свойствам динамической системы (размерность множества
$M$, эргодичность) можно получить информацию о слове $W$.

Важным примером в изучении сверхслов динамическим подходом
являются слова с предельной функцией роста.

Хорошо известно, что если функция роста слова $V(n)$ (то есть
размерность пространства, порожденного словами степени не выше
$n$) при нектором $n$ удовлетворяет неравенству $V(n)<n(n+3)/2$,
то алгебра имеет линейный рост.

В работе Колотова \cite{Kol} \label{Kol} построены алгебры с
``предельной'' функцией роста (то есть когда $V(n)=n(n+3)/2$),
которые описаны в терминах поворота окружности. А именно, все
такие алгебры, кроме счетного множества, строятся как алгебры
$A_W$, где $W=\{w_i\}$ -- слово над алфавитом $\{0,1\}$,
задаваемая иррациональными $\alpha,\beta\in (0,1))$:
$w_i=f(i+1)-f(i)$, где $f(i)=[\alpha i + \beta]$. В комбинаторике
слов чаще под функцией роста понимается функция $T(n)$ -
количество различных подслов длины $n$. И, таким образом,
$V(n)=\sum_{k}T_k$.

Слова с предельной функцией роста $T(n)=n+1$ образуют класс так
называемых {\it слов Штурма (Sturmian words)}, другое название --
{\it слова Бетти (Beaty words)}, которые впервые были упомянуты в
работе \label{HedlundMorse} \cite{MorseHedlund} Hedlund, Morse
``Symbolic dynamics II. Sturmian trajectories''.

Классическая теория слов Штурма описана в обзорах
\label{BerstelSeebold} \cite{BS}, \cite{AdL}.

К наиболее важным результатам в теории слов Штурма относится так
называемая {\it теорема эквивалентности}, в которой утверждается
эквивалентность трех классов сверхслов над двубуквенным алфавитом:
\begin{theorem}\label{TheorEq}
Следующие условия на слово $W$ эквивалентны:
\begin{enumerate}
\item Слово $W$ имеет фунцию сложности $T_W(n)=n+1$.

\item Слово $W$ сбалансированно и непериодично.

\item Слово $W$ порождается системой $(\mathbb{S}^1, U, T_\alpha)$
с иррациональным углом вращения $\alpha$.
\end{enumerate}
\end{theorem}

Последние продвижения в теории слов Штурма описаны в обзоре
\label{BerstelRecent} \cite{B} J. Berstel ``Recent results in
Sturmian words''.

Естественными обобщениями слов Штурма являются слова с минимальным
ростом, то есть слова с функцией роста $T(n)=n+K$, начиная с
некоторого $n$. Для двубуквенных алфавитов они носят название {\it
квазиштурмовых} слов. Слова с функцией роста, удовлетворяющей
соотношению $\lim_{n \to \infty} T(n)/n = 1$ изучены в работе
\label{Aberkane} \cite{Ab} A.Aberkane ``Words whose complexity
satisfies $\lim p(n)/n = 1$''.

Другим обобщением слов Штурма является обобщение, связанное с
понятием {\it сбалансированности}, а также {\it
$m$-сбалансированности}. Сбалансированные непериодические слова
над $n$-буквенным алфавитом изучены в работе \label{Graham}
\cite{GR} Graham ``Covering the Positive Integers by disjoints
sets of the form $\{n\alpha + \beta\}:n=1; 2;\ldots$''. Построение
порождающей динамической системы для сбалансированных
непериодических слов является одним из результатов данной работы.

Описание периодических сбалансированных слов связано с {\it
гипотезой Френкеля (Fraenkel's conjecture)}, утверждающей, что все
сбалансированные периодические слова над алфавитом
$A=\{a_1,\ldots, a_n\}$ из $n$ символов имеют вид

$$
W=(U_n)^{\infty},
$$
где $U_n$ задается рекуррентно:
$$
U_n=(U_{n-1}a_nU_{n-1}), \ U_3=a_1a_2a_1a_3a_1a_2a_1.\\
$$
Для 3-х буквенного алфавита гипотеза была доказана Р. Тайдеманом
(\cite{T1,T2}). В настоящий момент гипотеза доказана для алфавитов
состоящих не более чем из $7$ символов.


%Важным инструментом при описании сверхслов с различными
%комбинаторными свойствами является понятие графов подслов или
%графов Рози. Если $W$ - бесконечное сверхслово над алфавитом $A$,
%то $k$- графом Рози называется граф, вершины которого соответсвуют
%различным подсловам $W$ длины $k$. Из вершины $w_1$ в вершину
%$w_2$ ведет стрелка, если максимальный суффикс $w_1$ совпадает с
%максимальным префиксом $w_2$, то есть $w_1=a_1u$, $w_2=ua_2$, где
%$a_1,a_2 \in A$.

Продвижение в задачах символической динамики для слов с линейной
функцией роста получено в работе \cite{AR} \label{ArnouxRazy}
Arnoux, Rauzy "Representation geometrique des suites the
complexite $2n + 1$". В этой работе построена динамическая система
для слов с функцией роста $T(n)=2n+1$, обладающих дополнительным
комбинаторным свойством. В работе \label{Rote} \cite{R} G.Rote,
``Sequences with subword complexity 2n'' в терминах эволюции
графов Рози описаны слова с функцией роста $2n$.

Одним из основных результатов данной работы является обобщение
этих результатов на слова c линейной функцией роста, то есть с
функцией роста $T(n)=kn+l$, для $n>N$.

\subsection {Цель работы.} Данная диссертация посвящена
построению примеров динамических систем, порождающих различные
обобщения слов Штурма, в том числе над многобуквенными алфавитами.

\subsection{Научная новизна.}
Все основные результаты являются
новыми. Среди них можно отметить следующие:

\begin{enumerate}
\item Построение динамической системы для  сбалансированных
непериодических слов над произвольным алфавитом.

\item Построение динамической системы для произвольного
рекуррентного слова с минимальной функцией роста $T(n)=n+K$, для
$n>N$.

\item Построение общего критерия порождаемости слова
преобразованием перекладывания отрезков.

\end{enumerate}

\subsection{Основные методы исследования}

Основными инструментами исследования в работе являются различные
результаты теории слов Штурма, в частности теорема
эквивалентности. Для построения динамической системы, порождающей
сбалансированные слова используется лемма Кронекера-Вейля об
иррациональных сдвигах тора. Основным инструментом при изучении
слов медленного и линейного роста является рассмотрение эволюции
графов Рози.


\subsection{Практическая и теоретическая ценность}

Работа носит теоретический характер. Результаты диссертации могут
быть полезны в комбинаторной теории колец и полугрупп, в
частности, при изучении мономиальных алгебр, а также в
символической динамике.


\subsection{Краткое содержание работы}
{\bf Первая глава} посвящена обзору и доказательству базовых
результатов комбинаторики слов.

Отдельно рассматриваются результаты теории слов Штурма,
представлено доказательство теоремы эквивалентности, которое
используется в следующих главах.

Также доказываются основные результаты из теории графов Рози.

{\bf Вторая глава} посвящена изучению сбалансированных слов над
произвольным алфавитом. Изучаются свойства слов, порождаемых
иррациональными сдвигами тора.

Пусть $W$ -- слово над бинарным алфавитом, порождаемое сдвигом
одномерного тора, то есть динамикой
$(\mathbb{S}^1,U,T_\alpha,x_0)$.

Обозначим $\beta =\alpha/q+r/q$, $U_q=\{x|qx\in U\}$, $y_0=x_0/q$,
где $q$, $r$~--- целые. Несложно показать, что динамика
$(\mathbb{S}^1,T_{\beta},U_q,y_0)$ порождает то же слово $W$.
Переход от первой динамики ко второй мы назовем {\it
$q$--размножением}

Доказана следующая теорема об эквивалентности динамик:

\begin{theorem}
Пусть два слова $W_1$ и $W_2$ порожденные динамиками
$(\mathbb{S}^1,T_{\alpha},U,x_0)$ и
$(\mathbb{S}^1,T_{\beta},V,y_0)$ совпадают. Тогда существуют $p$ и
$q$ такие, что множества $U$ и $V$ при соответствующих
размножениях совпадают c точностью до поворота,т.е.
$U_p=T_{\delta}(V_q)$ для некоторого $\delta$.
\end{theorem}

Далее проводим редукцию от сбалансированного слова $W$ над
$n$-~буквенным алфавитом к $n$ бинарным словам Штурма:

Построим слова $W_1,W_2, \ldots ,W_n$ над бинарными алфавитами

$$A_1=\{a_1,\bar{a_1}\}, A_2=\{a_2,\bar{a_2}\}, \ldots
,A_n=\{a_n,\bar{a_n}\}$$ следующим образом:

$W_i=(w^i_n)_{n\in\mathbb{Z}}$

$$
w^i_n=w_n=\left\{
\begin{array}{rcl}
   a_i, w_n=a_i\\
   \bar{a_i}, w_n \neq a_i\\
\end{array}\right.
$$

Каждому слову $W_i$ соответствует одномерная динамика
$(\mathbb{S}^1,T_{\alpha_i},\Delta_i, x_i)$, ее порождающая,
следовательно слово $W$ порождается свигом на $n$-мерном торе с
вектором сдвига $\gamma=(\alpha_1,\ldots \alpha_n)$.

Обозначим через $M$ замыкание траектории начальной точки
$x=~(x_1,x_2,\ldots, x_n)$ при действии $T_\gamma$.

Доказана следующая предложение:

\begin{proposition}
$M$ гомеоморфно множеству $\mathbb{S}^1\times \{1,2,\ldots ,N\}$.
\end{proposition}

Теперь видно, что динамика реализуется на множестве \par
$M=\mathbb{S}^1\times\{1,2,\ldots N\}$, а отображение имеет
вид:\par
$f:(x,k)\to (x+\alpha, k+1 \mod N)$. \par Будем теперь
понимать под $U_i$ характеристическое множество для символа $a_i$,
которое лежит на замыкании траектории, и пусть также $U^k_i$
обозначает часть характеристического множества, которое лежит на
$k$-ой компоненте связности (окружности) $M$. Далее изучаются
соответствующие характеристические множества.

Основным результатом данной главы является
\begin{theorem}
Пусть $W$-- сбалансированное непериодическое слово над алфавитом
$A$. Тогда для $W$ существует динамическая система $(M,f)$,
удовлетворяющая следующим условиям:
\begin{enumerate}
\item $M=\mathbb{S}^1 \times {\mathbb Z}_m$ как топологическое
пространство.

\item $f:M \to M$ есть композиция поворота на $\alpha$ в
$\mathbb{S}^1$ и сдвига на $1$  в ${\mathbb Z}_m$. Длина
$\mathbb{S}^1$ равна $m$.

\item Каждая компонента $\mathbb{S} \times \{k\}$ $k=1, \ldots ,n$
разбита на $2m$ дуг: $m$ красных и $m$ синих; все красные имеют
длину $\alpha$, все синие $1-\alpha$,красные и синие дуги
чередуются.

\item Синий цвет имеет $l$ оттенков, красный -- $k$ оттенков,
$k+l=|A|$-- число букв в алфавите. Все середины дуг даного оттенка
образуют вершины правильного многоугольника (``правильный
$1$-угольник'' -- это точка на окружности,``правильный
$2$-угольник'' -- пара диаметрально противоположных точек).

\item При переходе от компоненты $\mathbb{S} \times \{k\}$ к
компоненте $\mathbb{S} \times \{k+1\}$ ( $\mathbb{S} \times
\{m+1\}=\mathbb{S} \times \{1\}$) порядок расположения оттенков
внутри красных и синих компонент сохраняется, а сами красные и
синие дуги (``рулетки'') проворачиваются относительно друг друга
на $1$. Так что преобразование $f$ приводит к смещению на $\alpha$
относительно красных компонент и на $1-\alpha$ (в обратную
сторону) относительно синих.

\end{enumerate}
\end{theorem}


{\bf Третья глава} посвящена другому обобщению слов Штурма --
словам {\it медленного роста}. Слово $W$ называется {\it словом
медленного роста}, если $F_W(n)=n+K$, для всех $n\geq N$. В словах
Штурма $F_W(n)=n+1$ и $F_W(n+1)-F(n)=1$. Естественным обобщением
будут слова, для которых $F(n)=n+K$, то есть выполняется
$F(n+1)-F(n)=1$ для достаточно больших $n$.

Показывается, что для каждого такого слова существует граф Рози,
соответствующий некоторому слову Штурма. Действительно, если
начиная с некоторого $n>N$ выполняется $T(n)=n+K$, то это
означает, что для каждого $n>N$ в слове $W$ существует только одно
правое и одно левое специальное слово длины $n$. То есть в графах
Рози таких слов есть одна входящая и одна выходящая развилка, а
значит, существует слово Штурма с такой же эволюцией $k$-графов,
что и данное. Дальше просходит редукция к теореме эквивалентности.
Доказана следующая
\begin{theorem}\label{MinGrow}
Пусть $W$ -- рекуррентное слово над произвольным конечным
алфавитом $A$. Тогда следующие условия на слово $W$ эквивалентны:
\begin{enumerate}

\item Существует такое натуральное $N$, что функция роста слова
$W$ равна $T_W(n)=n+K$, для $n\geq N$  и некоторого постоянного
натурального $K$.

\item Существуют такое иррациональное $\alpha$ и целые $n_1,n_2,
\ldots n_m$, что слово $W$ порождается динамической системой
$(\mathbb{S}^1,T_\alpha, I_{a_1},\ldots ,I_{a_n},x)$, где
$T\alpha$ -- сдвиг окружности на иррациональную величину $\alpha$,
$I_{a_i}$ -- объединение дуг вида $(n_j\alpha,n_{j+1}\alpha)$.
\end{enumerate}
\end{theorem}

В четвертой главе используются обобщения результатов третьей главы
на слова с функцией роста $T_W(n)=kn+l$. Если слово обладает такой
функцией роста, то $T_W(n+1)-T_W(n)=k$.

Известно, что если перекладывание $k$ отрезков {\it регулярно}, то
есть траектория любого из концов отрезков перекладывания не
попадает на другой конец любого отрезка, то эволюция любой точки
является словом с ростом $T_W(n)=kn+l$.

Мы ищем условия на слово $W$, при которых оно порождалось бы
преобразованием перекладываний отрезка. Отметим, что сдвиг
окружности, по сути, является перекладыванием двух отрезков с
сохранением ориентации.

Доказана следующая
\begin{theorem}
Если слово $W$ порождается переклаыванием отрезка, то все его
специальные слова имеют валентность $2$. Эквивалентно, его графы
Рози имеют входящие и выходящие развилки степени $2$ (Первое
условие порождаемости слова перекладыванием отрезков).
\end{theorem}

Перед тем как сформулировать второе необходимое условие, покажем,
как будем строить соответствующее преобразование. На первом этапе
мы будем строить кусочно-непрерывное преобразование отрезка, из
которого потом построим собственно перекладывание.

При первой итерации мы разбиваем отрезок произвольным образом на
отрезки, которые соответствуют соответствующим символам. Для
построение отображения нам достаточно определить траекторию этих
точек и затем из соображений рекуррентности продолжить по
непрерывности на весь отрезок.

Отметим, что если рост слова имеет вид $T(n)=kn+l$, то при каждой
итерации у нас должно появляться ровно $k$ новых точек, которые
некоторым образом делят отрезочки, соответствующие специальным
словам (или развилкам в графах Рози).

Если в $k$-графе отсутствуют двойные развилки, соответствующие
биспециальным словам, то выбор точек деления происходит корректно
и произвольно. Если же двойные развилки есть, то при переходе к
графу последователя необходимо удалить какие-то ребра, чтобы
сохранить условие $1$ теоремы 1.5.

Изучены два случая: в первом мы предполагаем, что преобразование
не должно менять ориентацию отрезков, во втором случае смена
ориентации происходит произвольным образом.

Далее, в каждом графе для удобства для каждой исходящей развилки
мы можем определить красное и синее исходящее ребро (определим,
что красное идет к синему против часовой, минуя входящие ребра),
аналогично можно определить красное и синее входящие ребра.
Естественно, ребро может быть красным исходящим и синим входящим
одновременно. Соответственно по графам Рози можно определить
красные и синие специальные слова. Выбор удаляемых ребер связан со
сменой ориентации. Для первого случая доказана

\begin{theorem}
Чтобы равномерно-рекуррентное слово $W$ порождалось
перекладыванием отрезка с сохранением ориентации, необходимо и
достаточно
\begin{enumerate}
\item Все правые и левые специальные слова  имели валентность $2$.

\item Пусть $w$ -- произвольное биспециальное слово и слова
$a_iw,a_jw$ -- красное и синее левое специальные слова
соответственно,$wa_k, wa_l \in W$ -- красное и синее правое
специальное слова. Тогда запрещенными словами могут быть $a_jwa_k$
или $a_iwa_l$.
\end{enumerate}
\end{theorem}

Пусть $v,u$ -- биспециальные слова и $v \subset u$. Назовем в
таком случае $u$ -- {\it наследником} $v$.

Выбор запрещенных ребер для вершин соответствующим $v$ и $u$ в
графах Рози назовем {\it соответственным} в том случае, что либо в
обоих случаях меняется ориентация, либо в обоих не меняется.

Тогда для случая сменой ориентации теорема формулируется таким
образом:

\begin{theorem}
Чтобы равномерно-рекуррентное слово $W$ порождалось
перекладыванием отрезка со сменой ориентации, необходимо и
достаточно, чтобы
\begin{enumerate}
\item Все правые и левые специальные слова  имели валентность $2$.

\item Существует $n$ такое что для всех биспециальных слов $w$
длины больше $n$ выбор запрещенных слов происходит согласованно с
потомками.
\end{enumerate}
\end{theorem}

